Conditional Synthetic Live and Spoof Fingerprint Generation

Large fingerprint datasets, while important for training and evaluation, are time-consuming and expensive to collect and require strict privacy measures. Researchers are exploring the use of synthetic fingerprint data to address these issues. This paper presents a novel approach for generating synthetic fingerprint images (both spoof and live), addressing concerns related to privacy, cost, and accessibility in biometric data collection. Our approach utilizes conditional StyleGAN2-ADA and StyleGAN3 architectures to produce high-resolution synthetic live fingerprints, conditioned on specific finger identities (thumb through little finger). Additionally, we employ CycleGANs to translate these into realistic spoof fingerprints, simulating a variety of presentation attack materials (e.g., EcoFlex, Play-Doh). These synthetic spoof fingerprints are crucial for developing robust spoof detection systems. Through these generative models, we created two synthetic datasets (DB2 and DB3), each containing 1,500 fingerprint images of all ten fingers with multiple impressions per finger, and including corresponding spoofs in eight material types. The results indicate robust performance: our StyleGAN3 model achieves a Fr\'echet Inception Distance (FID) as low as 5, and the generated fingerprints achieve a True Accept Rate of 99.47% at a 0.01% False Accept Rate. The StyleGAN2-ADA model achieved a TAR of 98.67% at the same 0.01% FAR. We assess fingerprint quality using standard metrics (NFIQ2, MINDTCT), and notably, matching experiments confirm strong privacy preservation, with no significant evidence of identity leakage, confirming the strong privacy-preserving properties of our synthetic datasets.

==> pkg.tex <==
% packages for regular (non-ACM) build


\usepackage{authblk}
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[margin=1in]{geometry}
\usepackage{amssymb,amsmath,amsthm,amsfonts}

\usepackage{xcolor}
\usepackage{soul} %yellow highlighting
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{makecell}
\usepackage[inline]{enumitem}
\usepackage{subcaption}
\usepackage{graphicx}
%\usepackage{backref}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{balance}
% \usepackage{textgreek}

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\usetikzlibrary{arrows,shapes,positioning,shadows,trees}

\tikzset{
  basic/.style  = {draw, text width=2cm, drop shadow, font=\sffamily, rectangle},
  root/.style   = {basic, rounded corners=2pt, thin, align=center,
                   fill=green!30},
  level 2/.style = {basic, rounded corners=6pt, thin,align=center, fill=green!60,
                   text width=8em},
  level 3/.style = {basic, thin, align=left, fill=pink!60, text width=6.5em}
}


\usepackage[pagebackref]{hyperref}
\hypersetup{
    colorlinks,
    linkcolor={red!50!black},
    citecolor={blue!50!black},
    urlcolor={blue!80!black},
    pdfstartview={XYZ null null 1.25}
}

\captionsetup{belowskip=4pt,aboveskip=1pt} %remove space after table caption




==> regauthors.tex <==

\newcommand{\clrksn}{{*}}
\newcommand{\afrl}{{$^{\ddagger}$}}

\renewcommand*{\Authsep}{\ }
\renewcommand*{\Authand}{\ }
\renewcommand*{\Authands}{\ }
%\setlength{\affilsep}{5em}

\author[\clrksn]{Syed Konain Abbas}
\author[\clrksn]{Sandip Purnapatra}
\author[\afrl]{Sarwar Murshed}
\author[\clrksn]{Conor Miller-Lynch} 
\author[\clrksn]{\authorcr Lambert Igene} 
\author[\clrksn]{Soumyabrata Dey} 
\author[\clrksn]{Stephanie Schuckers} 
\author[\clrksn]{Faraz Hussain} 
\affil[\clrksn]{Clarkson University, Potsdam, NY, USA\authorcr {\tt \{abbas,purnaps,millerlc,sdey,sschucke,fhussain\}@clarkson.edu}\vspace{0.4em}}
\affil[\afrl]{University of Wisconsin-Green Bay, WI, USA\authorcr {\tt murshedm@uwgb.edu}\vspace{0.4em}}


